Large Language Models are Temporal and Causal Reasoners for Video Question Answering

Large Language Models (LLMs) have shown remarkable performances on a wide range of natural language understanding and generation tasks. We observe that the LLMs provide effective priors in exploiting $\textit{linguistic shortcuts}$ for temporal and causal reasoning in Video Question Answering (VideoQA). However, such priors often cause suboptimal results on VideoQA by leading the model to over-rely on questions, $\textit{i.e.}$, $\textit{linguistic bias}$, while ignoring visual content. This is also known as `ungrounded guesses' or `hallucinations'. To address this problem while leveraging LLMs' prior on VideoQA, we propose a novel framework, Flipped-VQA, encouraging the model to predict all the combinations of $\langle$V, Q, A$\rangle$ triplet by flipping the source pair and the target label to understand their complex relationships, $\textit{i.e.}$, predict A, Q, and V given a VQ, VA, and QA pairs, respectively. In this paper, we develop LLaMA-VQA by applying Flipped-VQA to LLaMA, and it outperforms both LLMs-based and non-LLMs-based models on five challenging VideoQA benchmarks. Furthermore, our Flipped-VQA is a general framework that is applicable to various LLMs (OPT and GPT-J) and consistently improves their performances. We empirically demonstrate that Flipped-VQA not only enhances the exploitation of linguistic shortcuts but also mitigates the linguistic bias, which causes incorrect answers over-relying on the question. Code is available at https://github.com/mlvlab/Flipped-VQA.

==> Figures/tsne.tex <==
\begin{figure}[t] 
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/tsne.png}
    \caption{\textbf{T-SNE visualization.}
    We visualize the embedding space of language tokens and visual tokens (with and without $\mathcal{L}_\text{qav}$).
    }
    \label{fig:tsne}
\end{figure}

==> Tables/prior.tex <==
\begin{table}[t!]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{c|c|c|c c c c}
        \toprule
        \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Task}} & \multicolumn{4}{c}{\textbf{NExT-QA}} \\
        & & & Cau. & Tem. & Des. & Tot. \\
        \midrule
        \midrule
        \multirow{6}{*}{\textbf{LLaMA}} & \multirow{2}{*}{\textbf{7B}} & VQA & 67.8 (+0.0) & 65.6 (+0.0) & 71.9 (+0.0) & 68.7 (+0.0) \\
        & & QA & 51.7 (\textcolor{red}{-16.1}) & 52.3 (\textcolor{red}{-13.3}) & 46.8 (\textcolor{red}{-25.1}) & 51.1 (\textcolor{red}{-17.6}) \\
        \cmidrule{2-7}
        & \multirow{2}{*}{\textbf{13B}} & VQA & 69.5 (+0.0) & 66.5 (+0.0) & 72.8 (+0.0) & 69.1 (+0.0) \\
        & & QA & 54.1 (\textcolor{red}{-15.4}) & 53.8 (\textcolor{red}{-12.7}) & 49.4 (\textcolor{red}{-23.4}) & 53.3 (\textcolor{red}{-15.8}) \\
        \cmidrule{2-7}
        & \multirow{2}{*}{\textbf{33B}} & VQA & 72.6 (+0.0) & 67.1 (+0.0) & 73.7 (+0.0) & 71.0 (+0.0) \\
        & & QA & 57.4 (\textcolor{red}{-15.2}) & 56.0 (\textcolor{red}{-11.1}) & 50.8 (\textcolor{red}{-22.9}) & 55.9 (\textcolor{red}{-15.1}) \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Temporal and causal reasoning of LLaMA.}
    }
    \label{tab:prior}
\end{table}
